Fine-grained Recognition in the Wild: A Multi-Task Domain Adaptation Approach

While fine-grained object recognition is an important problem in computer vision, current models are unlikely to accurately classify objects in the wild. These fully supervised models need additional annotated images to classify objects in every new scenario, a task that is infeasible. However, sources such as e-commerce websites and field guides provide annotated images for many classes. In this work, we study fine-grained domain adaptation as a step towards overcoming the dataset shift between easily acquired annotated images and the real world. Adaptation has not been studied in the fine-grained setting where annotations such as attributes could be used to increase performance. Our work uses an attribute based multi-task adaptation loss to increase accuracy from a baseline of 4.1% to 19.1% in the semi-supervised adaptation case. Prior do- main adaptation works have been benchmarked on small datasets such as [46] with a total of 795 images for some domains, or simplistic datasets such as [41] consisting of digits. We perform experiments on a subset of a new challenging fine-grained dataset consisting of 1,095,021 images of 2, 657 car categories drawn from e-commerce web- sites and Google Street View.

==> acknowledgements.tex <==
We thank Kenji Hata, and Oliver Groth for their valuable feedback. This research is partially supported by an ONR MURI grant, the Stanford DARE fellowship (to T.G.) and by NVIDIA (through donated GPUs).te


==> dataset.tex <==
\tg{Make this section shorter}

\tg{Describe the office dataset and MNIST/SVHN dataset and more explicitly discuss why our dataset is much better than these for domain adaptation. I.e., larger-scale, more real world scenario etc...}

\tg{Word things such that it will go to the domain adaptation community who will appreciate the dataset}

A comprehensive study of visual domain adaptation has been limited by the relatively small scale of standard available datasets~\cite{office_dataset, crossdataset}. Here, we describe our fine-grained car dataset for domain-adaptation. Our dataset consists of $1,095,021$ images of $2,657$ categories of cars from $4$ sources: craigslist.com, cars.com, edmunds.com and Google Street View. We refer to images from craigslist.com, cars.com and edmunds.com as \textit{web} images and those from Google Street View as \textit{GSV} images. As shown in Fig.~\ref{fig:dataset_sources}, cars in \textit{web} images are large and typically unoccluded whereas those in \textit{GSV} are small, blurry and occluded. The difference in image size is apparent in Fig.~\ref{fig:dataset_bboxes} which shows a histogram of bounding box sizes in \textit{GSV} and \textit{web} images. These large variations in pose, viewpoint, occlusion and resolution make our dataset ideal for a study of domain adaptation. 

\textbf{Fine-Grained Car Categories.}
While the standard domain adaptation dataset~\cite{office_dataset} consists of $31$ types of objects, our large-scale car dataset consists of $2,657$ fine-grained car categories. This visually distinct set of cars comprises of nearly all cars in the US that were manufactured since 1990. As shown in Fig.~\ref{fig:fine-grained}, differences between some car classes can be almost imperceptible to an untrained expert. For example, the 2006 Honda accord sedan hybrid and the 2007 Honda accord sedan ex only differ in the appearance of their bumpers and trims. Our dataset is the first one to provide a benchmark for adaptation in the challenging fine-grained setting. 
\begin{figure}
%\includegraphics[width=\linewidth]{figs/fine-grained_cars.jpeg}
\includegraphics[width=\linewidth]{figs/fine-grained_one.pdf}
\caption{Two distinct classes of cars in our dataset. Some classes can differ by subtle changes in bumpers or trims. E.g., the 2005 Honda Accord sedan hybrid (\textit{left}) and the 2006 Honda Accord sedan hybrid (\textit{right}) differ by subtle changes in their trim and bumpers. The former has a plastic trim while the latter has a metal one.}
\label{fig:fine-grained}
\end{figure}
\begin{figure}
\includegraphics[width=\linewidth]{figs/bboxes.pdf}
\caption{Histogram of \textit{GSV} (left) and \textit{web} (right) bounding box sizes. While cars in \textit{GSV} images are typically small (with an average size of $9,117$ pixels), those in \textit{web} images are much larger, occupying an average of $146,848$ pixels.}
\label{fig:dataset_bboxes}
\end{figure}

\textbf{Annotation.}
Since our \textit{web} images are scraped from e-commerce websites, we collect labels for them by leveraging people looking to sell their cars. While these individuals are not car experts, they have detailed knowledge of the type of car they are selling. Thus, labels for \textit{web} images can be scraped from posts associated with each image and cleaned up using the amazon mechanical turk (AMT) user interface shown in Fig.~\ref{fig:annotation}. In contrast to \textit{web} images, in Google Street View we have no prior information regarding car categories in any particular image. Therefore, we hired experts to annotate these images using the user interface in Fig.~\ref{fig:annotation}. Only experts who could annotate at a speed of $1$ car per minute and a precision of at least $80\%$ were allowed to annotate our images. A total of $110$ expert human annotators worked for approximately two thousand hours to label our dataset. The distribution of annotated images across car classes is shown in Fig.~\ref{fig:label_dist}. While we have close to $900$ annotated \textit{web} images for popular cars such as the 2001-2003 Hyundai Elantra sedan gls, rare ones like the 1990-1992 Audi 80 sedan base have less than $10$ images. Similarly, due to the varying degrees of popularity and ease of recognition, GSV labels are not uniformly distributed. For instance, we have close to $500$ annotated images for the 2000-2006 Chevrolet Suburban SUV lt, and less than $5$ images for the 2012 Mercedes-Benz C Class sedan C63. 

%\vspace{-0.6cm}
\textbf{Car Metadata.}
In addition to the category labels, each class is accompanied by metadata listed below. These consist of the make of the car, of $58$ possible makes; the model of the car, of $777$ possible models; the year each car was manufactured; the body type of the car, of $11$ possible body types; the country of the car manufacturer, of $7$ possible countries; the typical miles per gallon of the car when driven on highways; the typical miles per gallon of the car when driven on non-highway streets; the price of the car in 2012. In our experiments, we use make, model and body type annotations. 

\begin{figure}
\includegraphics[width=\linewidth]{figs/annotation.jpeg}
\caption{\tg{might take out this figure.}Our annotation environment for \textit{GSV} (left) and \textit{web} images (right). Our \textit{GSV} user interface guides expert annotators by showing example images for each class. Our \textit{web} user interface asks annotators on Amazon Mechanical Turk (AMT) to only pick images showing exterior views of cars.}
\label{fig:annotation}
\end{figure}

%\begin{figure*}
%\includegraphics[width=\linewidth]{figs/label_dist.pdf}
%caption{The number of images for each of our $2,657$ classes for \textit{web} (left) and \textit{GSV} (right) classes. Some classes are more popular than others and are easier for experts to recognize. Thus, the distribution of images is not uniform.}
%\label{fig:label_dist}
%\end{figure*}







==> table_domain_shift.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{lccccc}
\toprule
\textbf{Training Data} & \textbf{Testing Data} & \textbf{Class Acc(\%)} & \textbf{Make Acc(\%)} & \textbf{Model Acc(\%)} & \textbf{Body Acc (\%)}\\
\midrule \midrule
Source & Source  & $73.9$ & $85.0$ & $82.2$ & $92.0$\\ 
Source & Target  & $8.5$  & $36.2$ & $18.2$ & $59.7$\\
Target & Target  & $18.9$ & $51.9$ & $31.6$ & $73.9$\\ %again we had 19.0 for target-->target 
%Target & Source  & $5.5$  & $41.4$ & $19.0$ & $60.3$ \\
%Source + Target  & Source & $75.5$ & $89.4$ & $81.7$ & $89.5$\\
Source + Target  & Target & $27.9$ & $56.4$ & $41.1$ & $75.8$\\
\bottomrule
\end{tabular}
\end{center}
\caption{We quantify the amount of domain shift between the \textit{web} source domain and \textit{GSV} target domain. We view the oracle in domain performance of training and testing on the source or target domains.
%All models are based on~\cite{alexnet}. Our source data consists of images from craigslist.com, cars.com and edmunds.com and our target images consist of Google Street View images. 
Accuracies are shown for models trained at the fine-grained class, make, model and body-type level. There are $170$ fine-grained classes, $89$ models, $17$ makes and $10$ body-types in our dataset.}
\label{table:domain_shift}
\end{table*}

==> table_main_result.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Dataset} & \textbf{Acc Baseline(\%)} & \textbf{Ours--Acc Multitask (\%)}\\
\midrule\midrule
\fbox{\textbf{Unsupervised Target}}& &  \\
Source CNN   & Cars & $8.6$ & $\textbf{13.7}$\\ 
Domain Confusion~\cite{tzeng2015iccv} & Cars & $14.17$ & $\textbf{18.0}$\\
%Gradient Reversal~\cite{gradient_reversal}& Cars & $\todo{X}$ &$\todo{X}$\\
Source CNN   & Office~\cite{office_dataset} & $\textbf{60.09}$ & $59.86$\\ 
Domain Confusion~\cite{tzeng2015iccv} & Office~\cite{office_dataset} & $61.06$ & $\textbf{62.4}$\\
%Gradient Reversal~\cite{gradient_reversal}&Office~\cite{office_dataset} & $\todo{X}$ &$\todo{X}$\\
\midrule\midrule
\fbox{\textbf{Semi-supervised Target}}\\
Source + Target (Subset) CNN & Cars & $3.4$ & $\textbf{7.2}$\\
Domain Confusion + Softlabel~\cite{tzeng2015iccv} & Cars & $12.0$ & $\textbf{19.0}$\\
Source + Target (Subset) CNN  & Office~\cite{office_dataset}  & $\textbf{45.5}$ & $45.2$\\
Domain Confusion + Softlabel~\cite{tzeng2015iccv} & Office~\cite{office_dataset}& $47.0$ & $\textbf{51.75}$\\
%\midrule\midrule
%\fbox{\textbf{Supervised Target}}\\
%Target CNN & Cars & $18.9$ & 15.8\\ 
%Source + Target CNN (FG) & Web + GSV (all) & 27.9 & 25.9\\
%Source + Target CNN (FG) + DC  & Web + GSV (all) & \bf 29.2 & \bf 28.9\\
\bottomrule
\end{tabular}
\end{center}
\caption{\todo{break acc down by acc (all) and acc (heldout), copy more numbers from excel table}Fine-grained classification accuracy for all (170) and held-out (85) classes with our final model as well as various baselines. Source CNN (FG) is a model trained only with source (\textit{web}) images and fine-grained class labels. DC refers to domain confusion loss. While GSV refers to \textit{GSV} images for all classes, GSV (subset) denotes labeled \textit{GSV} images for a subset, 85, of our 170 classes used during training. Softlabel is the soft label loss described in~\cite{tzeng2015iccv}. (FG) denotes models trained using only fine-grained labels, and (attributes) refers to the addition of independent attribute classifiers. Our model outperforms baselines in both the unsupervised and semi-supervised settings.}
\label{table:main_results}
\end{table*}










